Distortion Bounds of Subdivision Models for SO(3)

In the subdivision approach to robot path planning, we need to subdivide the configuration space of a robot into nice cells to perform various computations. For a rigid spatial robot, this configuration space is $SE(3)=\mathbb{R}^3\times SO(3)$. The subdivision of $\mathbb{R}^3$ is standard but so far, there are no global subdivision schemes for $SO(3)$. We recently introduced a representation for $SO(3)$ suitable for subdivision. This paper investigates the distortion of the natural metric on $SO(3)$ caused by our representation. The proper framework for this study lies in the Riemannian geometry of $SO(3)$, enabling us to obtain sharp distortion bounds.

==> Makefile <==
# file: Makefile-simple
#
# 	stand alone version (for papers)
# 	But prefix targets with "l" to avoid conflict.
#

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# file name:
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
p=p
p=question
p=ima2025-tmp
p=ima2025
p=ima2025-arxiv

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# software variants:
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
-include ~/bin/make-include

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# default:
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
default1: 2

default2: vi

what:
	-@echo "0 	=> pdflatex ima2025-tmp.tex"
	-@echo "1 	=> pdflatex ima2025.tex => ima2025-submit.pdf"
	-@echo "2 	=> pdflatex ima2025.tex => ima2025-arxiv.pdf"
	-@echo "acc0 	=> sumatraPDF ima2025-tmp.pdf"
	-@echo "acc1 	=> sumatraPDF ima2025-submit.pdf"
	-@echo "arxiv 	=> create ima2025-arxiv.zip "

0:
	make p=ima2025-tmp

1 ima2025-submit:
	-@echo "% file tmp-ifarxiv: auto-generated by Makefile" \
	        > tmp-ifarxiv.tex
	-@echo "% 	It must be included by p.tex" \
			>> tmp-ifarxiv.tex
	-@echo "\renewcommand{\ifarxiv}[2]{#2}" >> tmp-ifarxiv.tex
	make p=ima2025 pdf
	cp ima2025.pdf ima2025-submit.pdf

2 ima2025-arxiv:
	-@echo "% file tmp-ifarxiv: auto-generated by Makefile" \
	        > tmp-ifarxiv.tex
	-@echo "% 	It must be included by p.tex" \
			>> tmp-ifarxiv.tex
	-@echo "\renewcommand{\ifarxiv}[2]{#1}" >> tmp-ifarxiv.tex
	make p=ima2025-arxiv pdf
	cp ima2025-arxiv.pdf ima2025-arxiv-submit.pdf


acc0 accTmp:
	make acc p=ima2025-tmp

acc1 accIma:
	make acc p=ima2025-submit

acc2 accArxiv:
	make acc p=ima2025-arxiv

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# PDFLATEX:
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# Surf8:
pdflatex pdf: 
	$(PDFLATEX) ${p}.tex
	while [[ `cat ${p}.log | \
	    grep "Rerun to get cross"` ]] ; do \
	    echo "+++++++++ RERUN LATEX ++++++++++\n"; \
	    $(PDFLATEX) ${p}.tex; \
	  done

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# 	BIBTEX
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
bib ${p}.bbl:
	$(BIBTEX) ${p}

# works for Surf6:
bibtex:
	bibtex ${p}

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# 	Editor
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
vi:
	$(GVIM) $(p).tex &

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# 	PDFVIEWER
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
lview:
	myv ${p}.pdf &

# acrobat
acc:
	$(PDFVIEWER) -zoom 125%  ${p}.pdf &

# evince
ev evince:
	$(EVINCE) $(p).pdf &

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# Zipping for final submission to IMA and to arxiv
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

# Putting myTexmf files into arxivFolder:
#		svproc.cls,
#		myMac-llncs.sty, mac-robot.tex, lmac-robot.tex
arxivPrep:
	-rm -r arxivFolder/*
	cp ~/mac/mac/{svproc.cls,myMac-llncs.sty} arxivFolder
	cp ~/mac/mac/{mac-robot.tex,lmac-robot.tex} arxivFolder
	cp ima2025-arxiv-sav.bbl  ima2025-arxiv.bbl

# this creates ima2025-arxiv.zip for submission to arXiv:
zipArxiv arxiv: arxivPrep ima2025-arxiv
	cp ima2025-arxiv-submit.pdf  arxivFolder
	cp -r \
			ima2025-arxiv.tex \
			figs \
			Makefile lmac.tex\
			p1-intro.tex \
			p2-distort.tex \
			p3-reduction.tex \
			p5-conclud.tex \
			ima2025-arxiv-sav.bbl \
			tmp-ifarxiv.tex \
		arxivFolder
	-rm -f ima2025-arxiv.zip; 
	zip -r ima2025-arxiv.zip \
		arxivFolder

imaPrep:
	-rm -r imaFolder/*
	cp ~/mac/mac/{svproc.cls,myMac-llncs.sty} imaFolder
	cp ~/mac/mac/{mac-robot.tex,lmac-robot.tex} imaFolder

# this creates ima2025-submit.zip for submission to IMA proceedings:
zipIMA: imaPrep ima2025-submit
	cp README-ima imaFolder/README
	cp ima2025-submit.pdf imaFolder/ima2025-yapZhang.pdf
	cp -r ima2025.tex \
			Makefile \
			figs \
			lmac.tex \
			p1-intro.tex \
			p2-distort.tex \
			p3-reduction.tex \
			p5-conclud.tex \
			ima2025-small-sav.bbl \
		imaFolder
	-rm -f ima2025-submit.zip
	zip -r ima2025-submit.zip \
		imaFolder

#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
# Bookkeeping, one-time
#%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
m:
	${GVIM} Makefile &

spell:
	aspell -c xinc.tex

xinc:
	cp p1-intro.tex xinc.tex
	cat p2-distort.tex >> xinc.tex
	cat p3-reduction.tex >> xinc.tex
	cat p5-conclud.tex >> xinc.tex

postIMA:
	cp ima2025-submit.zip ima2025-submit-14may25.zip
	cp ima2025-submit-14may25.zip tmp
	cp ima2025-submit-14may25.zip ~/Uploads/2pdf/

postArxiv:
	cp ima2025-arxiv.zip ima2025-arxiv-14may25.zip
	cp ima2025-arxiv-14may25.zip ~/Uploads/2pdf/
	cp ima2025-arxiv-14may25.zip tmp

ln:
	-ln -s p1-intro.tex 1.tex
	-ln -s p2-distort.tex 2.tex
	-ln -s p3-subdiv.tex 3.tex
	-ln -s p4-adjacency.tex 4.tex
	-ln -s p5-conclud.tex 5.tex
	-ln -s p6-appendix.tex 6.tex
	-ln -s p7-supplement.tex 7.tex
	-ln -s p8-latestProof.tex 8.tex

######################################################
# END
######################################################


